Differentially Private Continual Release of Graph Statistics

Motivated by understanding the dynamics of sensitive social networks over time, we consider the problem of continual release of statistics in a network that arrives online, while preserving privacy of its participants. For our privacy notion, we use differential privacy -- the gold standard in privacy for statistical data analysis. The main challenge in this problem is maintaining a good privacy-utility tradeoff; naive solutions that compose across time, as well as solutions suited to tabular data either lead to poor utility or do not directly apply. In this work, we show that if there is a publicly known upper bound on the maximum degree of any node in the entire network sequence, then we can release many common graph statistics such as degree distributions and subgraph counts continually with a better privacy-accuracy tradeoff. Code available at https://bitbucket.org/shs037/graphprivacycode

==> metaalgoffline.tex <==
\section{The Main Algorithm}

We now consider the main problem of this paper. We are given a $D$-bounded graph sequence $\calG = ( G_1, G_2, \ldots )$, a privacy parameter $\epsilon$ and a function $f$ and our goal is to publish an approximation to the sequence $f(\calG)$. We also assume that the graph sequence arrives in an online manner as nodes get added; this implies that at time $t$, we only have access to $(G_1, G_2, \ldots, G_t)$. 

A naive approach to this problem is as follows. For each $t$, calculate $f(G_t)$ and add noise proportional to the global sensitivity divided by $\epsilon$. Unfortunately, it so happens that for many popular functions $f$, the global sensitivity scales with $m$, the length of the entire graph sequence even if it is degree-bounded. For example, suppose $f(G)$ is the number of nodes in $G$ with degree $\geq \tau$. Here, a single extra node with degree $\geq \tau$, added at time $t=1$, can increase $f(G_t)$ by $1$ for {\em{every}} $t$, thus increasing the global sensitivity of the sequence by $m$. 

The main observation in this work is that for a lot of popular functions $f$, the {\em{difference sequence}} $( f(G_1), f(G_2) - f(G_1), f(G_3) - f(G_2), \ldots)$ has considerably less global sensitivity. In particular, we show that if the graph sequence $\calG$ is $D$-bounded, for a number of functions $f$, the global sensitivity $\GS{D}{\Delta}$ of the entire difference sequence depends only on $D$ and not on the sequence length $m$. For example, in Section~\ref{sec:highdeg}, we show that if $f$ is the number of nodes with degree $\geq \tau$, then the global sensitivity of the entire sequence is at most $2D + 1$ for $D \geq \tau$. 

This immediately suggests the following algorithm.  For each $t \geq 1$, calculate the difference sequence $(\Delta_t)$, and add Laplace noise proportional to its global sensitivity over $\epsilon$ to get a private perturbed version $\tilde{\Delta}_t$. Then, the partial sums $(\tilde{\Delta}_1, \tilde{\Delta}_1 + \tilde{\Delta}_2, \ldots )$ constitute an approximation to $f(\calG)$ Observe that at time $t$, we only need to access the sequence $G_1, \ldots, G_t$, so the entire algorithm can be run online. Algorithm~\ref{alg} describes a general version of the algorithm, applied to a generic function $f$.


\begin{algorithm}[H]
\KwIn{Graph sequence $\calG$, query $f$, privacy parameter $\epsilon$}
Calculate the difference sequence $(\Delta)$, where $\Delta_1 = f(G_1)$, $\Delta_t = f(G_t) - f(G_{t-1})$, for $t \geq 1$.\\ 
Let $\GS{D}{\Delta}$ be the global sensitivity of the difference sequence\;
Calculate $\tilde{\Delta}_t = \Delta_t + \Lap{\frac{\GS{D}{\Delta}}{\epsilon}}$, for $t=1, \ldots, m$.\\
\Return{$\{ \sum_{s=1}^{t} \tilde{\Delta}_s \}_{t=1}^m$}
\caption{Main algorithm for publishing a function of a graph sequence}
\label{alg}
\end{algorithm}

The rest of the paper is devoted to analyzing the global sensitivity of the difference sequence for a number of popular functions $f$, and showing that it is independent of $m$.

\kc{One thing that does not come across -- what about composition? Think about how to write this properly.}



==> untitled folder/algorithms.tex <==
\section{Functions of Degree Distributions}\label{sec:degree}
%
%

We begin with functions of the degree distributions of the graph sequence, and consider both directed and undirected graphs. 
%
%
%
A summary of the results in this section is provided in Table~\ref{tab:resultsdegree}.

%

\begin{table*}[h]
\centering
\caption{Summary of degree distribution results.}
\label{tab:resultsdegree}
\begin{tabular}{ l || c | c}
\hline
						&	Undirected graph					&	Directed graph	\\ \hline
(out-)degree histogram	&	$4D^2 + 2D + 1$ (for $D$-bounded)	&	$4\Dout\Din + 2\Dout + 1$ (for $(\Din, \Dout)$-bounded)			\\ \hline
high-(out-)degree nodes	&	$2D+1$ (for $D$-bounded)			&	$2\Din+1$ (for $\Din$-in-bounded)				\\ \hline
\end{tabular}
\vspace{-10pt}
\end{table*}


\subsection{Undirected Graphs}

For undirected graphs, we will consider two functions applied to graph sequences -- first, the number of nodes with degree greater than or equal to a threshold $\tau$, and second, the degree histogram. 

\subsubsection{Number of High Degree Nodes}\label{sec:highdeg}

Recall that $\highdegree{\tau}{G}$ is the number of nodes in $G$ with degree $\geq \tau$. We show below, that for $D$-bounded graphs, the difference sequence corresponding to $\highdegree{\tau}{G}$ has global sensitivity at most $2D+1$.

\begin{lemma}\label{lem:high-degree-undirected}
Let $f(G) = \highdegree{\tau}{G}$. For $D$-bounded graphs, the difference sequence corresponding to $f$ has global sensitivity at most $2D+1$. In fact, the global sensitivity is $2D+1$ for any $\tau < D$.
\end{lemma}
Notice that $\tau \leq D$ is needed for the statistic to be meaningful; if $\tau > D$, there is no high-degree node. 
%

%
%
%
%
%
%

%
%
%


\paragraph{Projection Yields High Sensitivity in Graph Sequence}
A common idea in static graph analysis with \nodeprivacy\ is to project the original graph into a bounded-degree graph. The sensitivity of some common statistics on this projected graph scales with the degree bound instead of the total number of nodes.
The current state-of-the-art projection algorithm is proposed in \cite{day2016publishing}. Given a projection threshold $\tD$, a graph $G = (V, E)$ and an ordering of the nodes in $V$, the algorithm constructs a bounded-degree graph $G^{\tD}$ as follows. First, it adds all nodes in $V$ to $G^{\tD}$; then it orders all edges in $E$ according to the ordering of $V$, and for each edge $(u,v)$, adds it to $G^{\tD}$ if and only if the addition does not make the degree of either $u$ or $v$ exceed $\tD$.

This algorithm can be easily adapted to the online graph setting. \showinlater{We give a complete description of the algorithm in Appendix~\ref{sec:appendix_baseline}}.
%
However, it can be shown that the global sensitivity of the difference sequence is proportional to the total number of publications. 

\begin{lemma}\label{lem:high-degree projection}
%
Let $f(G) = \highdegree{\tau}{G^{\tD}}$. For $D$-bounded graphs, the corresponding difference sequence that ends at time $T$ has global sensitivity at least $\tD T$ for any $\tD > \tau > 0$.
\end{lemma}
Notice that $\tD > \tau$ is needed for $\highdegree{\tau}{G^{\tD}}$ to be meaningful; otherwise, we would have $\highdegree{\tau}{G^{\tD}} = |V|$ for any $G$.


%

%
%

%

%
%
%

%


%
%
%
%
%
%
%
%


\subsubsection{Degree Histogram}
%
%
%
%
%
%
%
%
%
%
%
%
%
%

Degree histogram is another informative statistic of a graph. However, we can show that even for bounded graph, the sensitivity can scale quadratically with the degree bound. We use the generalized $L_1$ distance defined in Section~\ref{sec:notation} as the distance metric for the global sensitivity.

\begin{lemma}\label{lem:degree-hist undirected}
%
Let $f(G) = \hist{G}$. For $D$-bounded graphs, the difference sequence corresponding to $f$ has global sensitivity $4D^2 + 2D + 1$.
\end{lemma}
%


\subsection{Directed Graphs}
For Directed graphs, we show similar results for the number of nodes with out-degree greater than or equal to a threshold $\tau$ and the out-degree histogram. Similar results can be obtained for in-degree.

\subsubsection{Number of High Out-Degree Nodes}
Recall that $\highoutdegree{\tau}{G}$ denotes the number of nodes in $G$ with degree $\geq \tau$. We show below that for $\Din$-in-bounded graphs, the difference sequence corresponding to $\highoutdegree{\tau}{G}$ has global sensitivity $2\Din+1$.
\begin{lemma}\label{lem:high-degree-directed}
Let $f(G) = \highoutdegree{\tau}{G}$. For $\Din$-in-bounded graphs, the difference sequence corresponding to $f$ has global sensitivity $2\Din+1$.
\end{lemma}

%

\subsubsection{Out-Degree Histogram}
We show that for bounded directed graphs, the sensitivity of the histogram scales quadratically with the degree bounds as well.
\begin{lemma}\label{lem:out-degree-hist directed}
%
Let $f(G) = \histout{G}$. For $(\Din, \Dout)$-bounded graphs, the difference sequence corresponding to $f$ has global sensitivity $4\Dout\Din + 2\Dout + 1$. 
\end{lemma}


\input{algorithms_triangle}


==> untitled folder/algorithms_triangle.tex <==
\section{Functions of Subgraph Counts}\label{sec:subgraph}

In this section, we consider the count of some common directed and undirected subgraphs.

%
%

\paragraph{Popular subgraphs}
In undirected graphs, we consider three subgraphs. 1) an edge, including two nodes and the edge between them, 2) a triangle, including three nodes with edges between any two of them and 3) a $k$-star, including one center node $c$, $k$ boundary nodes $\{b_1,\dots,b_k\}$ and edges $\{(c,b_i):i\in[k]\}$. Table~\ref{tab:patterns_undirected} summarizes these subgraphs.

In directed graphs, we consider five subgraphs. 1) an edge, including two nodes and an directed edge between them, 2) triangle \rom{1}, including nodes $\{v_1,v_2,v_3\}$ and edges $\{(v_1,v_2),(v_2,v_3),(v_3,v_1)\}$, 3) triangle \rom{2}, including nodes $\{v_1,v_2,v_3\}$ and edges $\{(v_1,v_2),(v_1,v_3),(v_2,v_3)\}$, 4) an out-$k$-star, including one center node $c$, $k$ boundary nodes $\{b_1,\dots,b_k\}$ and edges $\{(c,b_i):i\in[k]\}$, 5) an in-$k$-star, including one center node $c$, $k$ boundary nodes $\{b_1,\dots,b_k\}$ and edges $\{(b_i,c):i\in[k]\}$.
Table~\ref{tab:patterns_directed} summarizes these subgraphs.

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\begin{table}[h]
\centering
\caption{Subgraphs in undirected graphs.}
\label{tab:patterns_undirected}
\begin{tabular}{ c | c | c}
Edge 		&	Triangle	&	$k$-star		\\\hline
$S^u_E$		&	$S^u_{\triangle}$		&	$S^u_{\star}$			\\\hline
\udedge 		&	\udtriangle &	$\udkstar{}$ 
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Subgraphs in directed graphs.}
\label{tab:patterns_directed}
\begin{tabular}{ c | c | c | c | c}
Edge 		&	Triangle \rom{1}	&	Triangle \rom{2}	 &	Out-$k$-star	&	In-$k$-star	\\\hline
$S^d_E$		&	$S^d_{\triangle^1}$	&	$S^d_{\triangle^2}$		&	$S^d_{\star^o}$	&	$S^d_{\star^i}$			\\\hline
\dedge 		&	\dtriangleI	&	\dtriangleII &	$\dkstarI{}$	&	$\dkstarII{}$ 
\end{tabular}
\end{table}



\subsection{Undirected Graphs}

First, we present a general result that applies to any undirected subgraph $S$. 
Recall that $\S{}{G}$ denotes the total number of copies of $S$ in graph $G$.
%
\begin{lemma}\label{lem:subgraph undirected}
%
Given any undirected subgraph $S$, if $\S{}{G}$ changes by at most $S_{+}$ with an additional node with degree $D$ (and the corresponding edges), then the difference sequence corresponding to $\S{}{\cdot}$ has global sensitivity $S_{+}$ for any $D$-bounded graph $G$.
\end{lemma}

Now we show the values of $S_{+}$ for the subgraphs listed in Table~\ref{tab:patterns_undirected}.
\begin{lemma}\label{lem:subgraph undirected patterns}
Given the degree bound $D$, the value of $S_{+}$ for some common subgraphs are:
\begin{enumerate}
\item for $S^u_E$,		$S_{+} = D$;
\item for $S^u_{\triangle}$, 	$S_{+} = {D \choose 2}$;
\item for $S^u_{\star}$, 	$S_{+} = D{D-1 \choose k-1} + {D \choose k}$.
\end{enumerate}
\end{lemma}


\subsection{Directed Graphs}

Again, we first present a lemma that applies to any subgraph $S$, and then show the values of $S_{+}$, the maximum change in the subgraph count caused by an additional node, for the subgraphs in Table~\ref{tab:patterns_directed}.
\begin{lemma}\label{lem:subgraph directed}
%
%
Given any directed subgraph $S$, if $\S{}{G}$ changes by at most $S_{+}$ with an additional node with $\Din$ in-degree and $\Dout$ out-degree (and the corresponding edges), then the difference sequence corresponding to $\S{}{\cdot}$ has global sensitivity $S_{+}$ for any $(\Din, \Dout)$-bounded graph $G$.
\end{lemma}

%
\begin{lemma}\label{lem:subgraph directed patterns}
Given degree bounds $\Din$ and $\Dout$, the value of $S_{+}$ for some common subgraphs are:
\begin{enumerate}
\item for $S^d_{E}$,		$S_{+} = \Din + \Dout$;
\item for $S^d_{\triangle^1}$, 	$S_{+} = \Din \Dout$;
\item for $S^d_{\triangle^2}$, $S_{+} = {{\Din + \Dout} \choose 2}$;
\item for $S^d_{\star^o}$, 	$S_{+} = \Din {\Dout - 1 \choose k - 1} + {\Dout \choose k}$;
\item for $S^d_{\star^i}$, $S_{+} = \Dout {\Din - 1 \choose k - 1} + {\Din \choose k}$.
\end{enumerate}
\end{lemma}


==> untitled folder/conclusion.tex <==
\section{Conclusion}
In summary, we present a general algorithm for continually releasing statistics
of a graph sequence.  Our proposed algorithm exploits the difference sequence
of the statistics, which has lower sensitivity compared to the original
sequence, to achieve improved utility.  We derive the global sensitivity of
the difference sequences for common statistics including degree statistics and
subgraph counts for bounded-degree graphs.  Evaluations on real and synthetic
graphs demonstrate the practical applicability of the proposed algorithm by
showing that it outperforms two natural baselines over a wide range of
parameters.  In particular, the proposed algorithm is much less sensitive with
respect to the number of releases compared with the baselines.  

Our work is thus a step towards privacy-preserving analysis of
online graphs, and has the potential to lead to insights in epidemiology of
stigma-inducing diseases such as HIV, while still preserving the patient
privacy.

%
%
%
%
%

%

%








==> untitled folder/experiments.tex <==
\section{Experiments}
We next demonstrate the practical applicability of the proposed algorithm by comparing it with some natural baselines. In particular, we investigate the following questions: \begin{enumerate}
\item What is the utility offered by \sensdiff\ as a function of the privacy parameter $\epsilon$ and the number of releases?
\item How does its utility compare with existing baselines, such as composition across time steps, and composition coupled with graph projection?
\end{enumerate}
These questions are considered in the context of five datasets -- two synthetic and three real online graphs. We consider two versions of each dataset -- directed and undirected, and two graph statistics -- the number of high-degree nodes and the number of edges. 


\subsection{Methodology}

\subsubsection{Baseline Algorithms}
We consider two natural baselines based on sequential differential privacy composition -- \composeD\ and \composeproj. \composeD\ considers each graph $G_t$ in the sequence separately, and adds noise to $f(G_t)$ that is proportional to its $D$-bounded global sensitivity divided by $\epsilon/T$. Here $\epsilon$ is the privacy parameter and $T$ is the number of releases. \composeproj uses a state-of-the-art projection algorithm -- the one proposed in \cite{day2016publishing} -- to project each $G_t$ into $\tilde{G}_t$, and releases $f(\tilde{G}_t)$ after adding noise proportional to its global sensitivity divided by $\epsilon/T$.

There are two other natural approaches. The first is to compute $f(\calG)$ and add noise proportional to its $D$-bounded global sensitivity divided by $\epsilon$; the second is to use the projection algorithm to obtain a sequence of projected graphs $\tilde{\calG} = (\tilde{G}_1,\dots,\tilde{G}_T)$, compute $f(\tilde{\calG})$ and add noise proportional to the its global sensitivity divided by $\epsilon$. However, we can show that the utility of either of these approaches is guaranteed to be at most that of \composeD\ and \composeproj; details are omitted due to space constraints.

%
%
%
%
%


\subsubsection{Choice of Parameters}
\sensdiff\ and \composeD\ both require an a-priori bound on the graph degree. We set this bound to be the actual maximum degree rounded up to the nearest $5$-th integer.

\composeproj\ requires a projection threshold $\tD$ (or, $\tDin$ and $\tDout$ for directed graphs). This parameter is chosen by parameter tuning -- we pick the parameter value out of a predetermined list that leads to the lowest error. Note that for the sake of fairness, we do not allocate any extra privacy budget to parameter tuning, which would be the case in reality; thus our estimate of the performance of \composeproj\ is {\em{optimistic}}. 
%
%
%
%
%
%
%
%
%
%
%

The threshold $\tau$ in the high-degree or high-out-degree nodes experiments is set to be the $90$-th percentile of the (non-private) degree distribution.

\subsection{Datasets}
We use five datasets -- three real and two synthetic. In addition to the standard directed version of each dataset, we also consider an undirected version that is obtained by ignoring the edge directions. A brief summary of these datasets is presented in Table~\ref{tab:data}.

\begin{table*}[h]
\centering
\caption{Summary of common properties of the graph datasets. Max degree refers to the undirected version of the graph while max in-degree and max out-degree refer to the directed version.}
\label{tab:data}
\begin{tabular}{ l || c | c | c | c | c | c}
\hline
					&	\# nodes	& \# edges	&	timespan (year)	&	max degree	&	max in-degree	&	max out-degree	\\ \hline
HIV transmission	&	$1660$	&$456$	&$21$	&$13$	&$12$	&$8$				\\ \hline
Patent citation		&$91614$	&$475427$	&$15$	&$247$	&$211$	&$246$	\\ \hline
Paper citation 		&$9038$	&$5249$	&$24$	&$36$	&$19$	&$36$	\\ \hline
Synthetic \rom{1}	&$1990$	&$665$	&$20$	&$5$		&$1$		&$4$	\\ \hline
Synthetic \rom{2}	&$1088$	&$588$	&$20$	&$6$		&$1$		&$5$	\\ \hline
\end{tabular}
\vspace{-0pt}
\end{table*}

\subsubsection{Real Data Sets}


\paragraph{HIV transmission graph} This is a graph of potential HIV transmissions where a node represents a patient and an edge connects two patients whose viral sequences have high similarity. An edge thus represents a plausible transmission; the graph also has spurious edges that may correspond to a patient transmitting the disease to multiple others within a short period of time. About two-thirds of the patients have an estimated date of infection (EDI) ranging from $1996$ to $2016$, which is taken as the time stamp of the corresponding node. For the remaining nodes, EDI could not be estimated as the patient was admitted long after infection; we set the corresponding time stamps as $1995$.

\paragraph{Patents citation graph} The patents citation graph \cite{data_patents} contains all US patents granted between $1963$ and $1999$, and all citations made by patents from $1975$ to $1999$. A patent $u$'s citing patent $v$ naturally yields a directed edge from $v$ to $u$. We pick all patents under subcategory {\em{Computer Hardware \& Software}} (indexed $22$) to form both a directed and an undirected graph, and publish statistics from years $1985$ to $1999$.

\paragraph{Paper citation graph} This is a graph of articles and their citations from ACL derived by~\cite{data_citation}; each article has a recorded publication date from $1975$ to $2013$. We select the positive citations, where an edge from $v$ to $u$ implies that $u$ endorsed the article $v$, and publish statistics from $1990$ to $2013$. 

\subsubsection{Synthetic Data Sets}

In addition to the real data sets, we consider two synthetic graphs that are generated from two separate disease transmission models.  


\def\BA{Barab\'asi--Albert}

\paragraph{Synthetic disease transmission graph \rom{1}}
This is a synthetic graph of disease transmissions based on the \BA\ preferential attachment model. In the \BA\ model, there are $m_0$ initial nodes, followed by a number of nodes that arrive sequentially. A node on arrival connects to $k$ existing nodes, with a higher chance of connecting to nodes with higher degree. 

We make three modifications to this model so that the generated graph is a more realistic disease transmission network. First, we
assume there is a total of $Y$ years with $n$ nodes added per year; each node has a time stamp -- its year of arrival -- and the initial nodes have time stamp $0$. All edges are directed from nodes with lower time stamps to those with higher time stamps.  Second, to model the large number of isolated nodes that exist in real disease transmission networks, we ensure that each new node is isolated with probability proportional to a parameter $P_{\text{isolated}}$. Third, in practice, an infected individual is usually less likely to spread infection as time passes due to treatment or death. We build this property into the model by adding an extra decaying factor to the connection probability, i.e., the probability of a new node's connecting to an existing node $v$ is proportional to $\degree{}{v} \times (\texttt{current\_time} - v.\time + 1)^{-c}$ (or $\outdegree{}{v} \times (\texttt{current\_time} - v.\time + 1)^{-c}$ in directed graph) where $c$ is the decay parameter. For our experiments, we generate a graph with parameters $P_{\text{isolated}} = 0.5$, $k = 1$, $m_0 = 500$, $n=70$, $Y=20$ and $c = 1$.



\paragraph{Synthetic disease transmission graph \rom{2}} This is a synthetic disease transmission graph drawn from the popular SIR model~\cite{SIRmodel} of infection overlaid on an underlying \BA\ social network. In the SIR model, a node or individual as three statuses -- susceptible (S), infectious (I) and recovered (R). The infectious individuals transmit the disease to susceptible individuals through social links with a transmission probability $P_t$. With probability $P_r$, an infectious individual can recover; once recovered, an individual will not get infected again.

%
We generate an undirected social network $G_{\text{interact}} = (V, E)$ from the \BA\ model, where a node represents a person and an edge a social interaction. We then simulate the transmission process as follows. Initially, every node is susceptible (S) except for $n_0$ randomly picked infectious (I) nodes. At time step $t$, an infectious node changes status to recovered (R) with probability $P_r$; then, each node $u$ that is still infectious infects each one of its neighbors in $G_{\text{interact}}$ with probability $P_i / \degree{G_{\text{interact}}}{u}$. This gives us a transmission graph where a directed edge is a disease transmission. The time stamp of each node is the time when it is infected. We note that any node in the social interaction graph that has never been infected will not appear in the transmission graph. For our experiments, we use the parameters $P_r = 0.1$, $P_i = 0.18$ and a underlying interaction graph $G_{\text{interact}}$ of size $10000$ with attachment parameter $k = 2$.


\subsection{Results}

\input{figures_layout}

We compare \sensdiff\ with the baseline algorithms \composeD\ and \composeproj\
under varying $\epsilon$ -- the privacy parameter and varying $T$ -- the number
of releases.  We measure utility by the relative $L_1$ error $\sum_{t=1}^T
\abs{\calA(G_t) - f(G_t)}/f(G_t)$, where $f(G_t)$ is the non-private statistic
and $\calA(G_t)$ is the value estimated by an algorithm.  

Figure~\ref{fig:epsilon} shows the privacy-utility tradeoffs of the three
algorithms for the number of high-degree nodes (1st and 2nd columns) and number
of edges (3rd and 4th columns) across all datasets (different rows).  There is
a clear trend of decreasing error as $\epsilon$ increases for all algorithms;
however, \sensdiff\ yields smaller error compared to the other two baselines in
all the cases. We point out that these results are overly optimistic for
\composeproj\ -- as we do not spend any privacy budget tuning the projection
thresholds.



Figure~\ref{fig:time} presents the utility of all algorithms across different datasets (different rows) and statistics (different columns) as a function of the number of releases $T$. We fix $\epsilon$ to be $5$.  We see that the relative error increases as $T$ increases for all algorithms, across all datasets and statistics. 
Similar to the previous experiment, \sensdiff\ achieves lower errors in most cases for the number of high-degree nodes and significantly lower errors in all cases for the number of edges. 
In addition, we observe that the error of \sensdiff\ increases at a smaller rate with increasing number of releases compared to the two baselines. This implies that \sensdiff\ achieves better utility for large $T$, and confirms the theoretical arguments in Section~\ref{sec:main_alg}. 

%
%


Reconsidering the two questions proposed in the beginning of the section, we conclude that \sensdiff\ offers better utility under a wide range of $\epsilon$ and $T$ compared to both baselines. \composeD\ yields the worst utility across all datasets for both statistics, which is to be expected as it does not take advantage of either projections or additional properties of the graph sequence. \sensdiff\ outperforms \composeproj\ in most cases, and has a more significant advantage for large $T$.



==> untitled folder/figures_layout.tex <==
\begin{table*}[!t]
\setlength\tabcolsep{0pt} %
\resizebox{\textwidth}{!}{
\begin{tabularx}{\textwidth}{c c c c c}
& Directed, high-degree & Undirected, high-degree & Directed, edge & Undirected, edge \\ 
\rotatebox[origin=l]{90}{\quad HIV transmission}
& \includegraphics[width=0.245\textwidth]{figure/hiv_directed_1_highDeg_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/hiv_undirected_1_highDeg_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/hiv_directed_1_edge_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/hiv_undirected_1_edge_cmp.pdf}
\\
\rotatebox[origin=l]{90}{\qquad Patent citation}
&\includegraphics[width=0.245\textwidth]{figure/patent_directed_1_highDeg_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/patent_undirected_1_highDeg_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/patent_directed_1_edge_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/patent_undirected_1_edge_cmp.pdf}
\\ 
\rotatebox[origin=l]{90}{\qquad Paper citation}
&\includegraphics[width=0.245\textwidth]{figure/citation-pos_directed_1_highDeg_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/citation-pos_undirected_1_highDeg_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/citation-pos_directed_1_edge_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/citation-pos_undirected_1_edge_cmp.pdf}
\\ 
\rotatebox[origin=l]{90}{\qquad \quad Synthetic \rom{1}}
&\includegraphics[width=0.245\textwidth]{figure/synth_BA_directed_1_highDeg_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_BA_undirected_1_highDeg_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_BA_directed_1_edge_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_BA_undirected_1_edge_cmp.pdf}
\\ 
\rotatebox[origin=l]{90}{\qquad \quad Synthetic \rom{2}}
&\includegraphics[width=0.245\textwidth]{figure/synth_SIR_directed_1_highDeg_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_SIR_undirected_1_highDeg_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_SIR_directed_1_edge_cmp.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_SIR_undirected_1_edge_cmp.pdf}\\
\end{tabularx}}
\captionof{figure}{$L_1$ error vs. privacy parameter $\epsilon$. Publish every $1$ year. Averaged over $100$ runs.}
\label{fig:epsilon}
\end{table*}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


\begin{table*}[!t]
\setlength\tabcolsep{0pt} %
\resizebox{\textwidth}{!}{
\begin{tabularx}{\textwidth}{c c c c c}
& Directed, high-degree & Undirected, high-degree & Directed, edge & Undirected, edge \\ 
\rotatebox{90}{\quad HIV transmission}
&\includegraphics[width=0.245\textwidth]{figure/hiv_directed_highDeg_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/hiv_undirected_highDeg_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/hiv_directed_edge_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/hiv_undirected_edge_eps5_time.pdf}
\\ 
\rotatebox{90}{\qquad Patent citation}
&\includegraphics[width=0.245\textwidth]{figure/patent_directed_highDeg_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/patent_undirected_highDeg_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/patent_directed_edge_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/patent_undirected_edge_eps5_time.pdf}
\\ 
\rotatebox{90}{\qquad Paper citation}
&\includegraphics[width=0.245\textwidth]{figure/citation-pos_directed_highDeg_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/citation-pos_undirected_highDeg_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/citation-pos_directed_edge_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/citation-pos_undirected_edge_eps5_time.pdf}
\\ 
\rotatebox{90}{\qquad \quad Synthetic \rom{1}}
&\includegraphics[width=0.245\textwidth]{figure/synth_BA_directed_highDeg_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_BA_undirected_highDeg_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_BA_directed_edge_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_BA_undirected_edge_eps5_time.pdf}
\\ 
\rotatebox{90}{\qquad \quad Synthetic \rom{2}}
&\includegraphics[width=0.245\textwidth]{figure/synth_SIR_directed_highDeg_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_SIR_undirected_highDeg_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_SIR_directed_edge_eps5_time.pdf}
& \includegraphics[width=0.245\textwidth]{figure/synth_SIR_undirected_edge_eps5_time.pdf}\\
\end{tabularx}}
\captionof{figure}{$L_1$ error vs. number of publications $T$. $\epsilon = 5$. Averaged over $100$ runs.}
\label{fig:time}
\end{table*}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


==> untitled folder/intro.tex <==
\section{Introduction}

%


Dynamic social networks are ubiquitous models of social and economic phenomena, and analyzing them over a period of time can allow researchers to understand various aspects of human behavior. Many social networks, however, include sensitive and personal information about the people involved. Consequently, we need to design privacy-preserving algorithms that can summarize properties of dynamic social networks over time while still preserving the privacy of the participants. 

As a concrete motivating example, consider data on HIV transmission collected from patients in a particular region over multiple years \cite{little2014using, wang2015targeting, wertheim2017social}. Advances in sequencing technology allow scientists to infer putative transmission links by measuring similarities between HIV sequences obtained from different patients. These links can then be resolved into transmission networks, reflecting the patterns of transmission  in that population. Epidemiologists would like to study properties of these networks as they grow over time to understand how HIV propagates. Since there is considerable social stigma associated with HIV, these networks are highly sensitive information, and public release of their properties needs to ensure that privacy of the included individuals is not violated. Additionally, analyses of these networks need to happen intermittently -- for example, once a year -- so that properties of the network as it evolves may be studied. %

In this paper, we consider continual privacy-preserving release of graph statistics, such as degree distributions and subgraph counts, from sensitive networks where nodes and their associated edges appear over time in an online manner. For our privacy notion, we use differential privacy~\cite{DMNS06} -- the gold standard in private data analysis. Differential privacy guarantees privacy by ensuring that the participation of a single person in the dataset does not change the probability of any outcome by much; this is enforced by adding enough noise to either the input data or to the output of a function computed on the data so as to obscure the private value of a single individual. Since in our applications, a node corresponds to a single person, we use node differential privacy~\cite{hay2009accurate}, where the goal is to hide the participation of any single node. 


There are two main challenges in continually releasing graph statistics with node differential privacy. The first is that node differential privacy itself is often very difficult to attain, and can only be attained in either bounded degree graphs or graphs that can be projected to be degree-bounded. The second challenge pertains to the online nature of the problem. Prior work has looked at continual release of statistics based on streaming tabular data~\cite{bolot2013private, cao2013efficient, chan2011private, kellaris2014differentially, chen2017pegasus, dwork2010differential}; however, these works rely on the fact that in tabular data, at any time $t$, we only get information about the $t$-th individual, and not about individuals who already exist in the data. This property no longer holds in online graphs, as an incoming node may bring in new information about existing nodes in the form of connecting edges, and therefore these solutions do not directly apply.

In this work, we show that if there is a publicly known upper bound on the maximum degree of any node in the entire graph sequence, then, a {\em{difference sequence}}  -- namely, the sequence of differences in the statistics computed on subsequent graphs -- has low sensitivity. The assumption of bounded maximum degree holds for many real networks, as many real-world graphs, such as 
social interaction networks, collaboration networks, computer networks and disease transmission networks, that are scale-free with power-law degree distributions have low maximum degree. Given this assumption holds, we show in particular that the sensitivity of the entire difference sequence only depends on the publicly known upper bound, and not on the length of the sequence. This implies that we can release a private version of the difference sequence with relatively high accuracy, which can be used to continually release the target statistic with high privacy-accuracy tradeoff. 

%
It is commonly believed that many real-world networks, such as social interaction networks, collaboration networks, computer networks and disease transmission networks are scale-free with degree distributions following a power law; such graphs have low maximum degrees.
%

We derive the sensitivity of the difference sequence for a number of common graph statistics, such as degree distribution, number of high degree nodes, as well as counts of fixed subgraphs. We then implement our algorithms and evaluate them on three real and two synthetic datasets against two natural baselines. Our experimental results show that the algorithm outperforms these baselines in terms of utility for these datasets over a range of privacy parameters.












%
%
%
%
%

%
%
%

%
%
%
%
%
%


%

\subsection{Related Work}

%

Since its inception~\cite{DMNS06}, differential privacy has become the gold standard for private data analysis and has been used in a long line of work -- see~\cite{SC13, DR14} for surveys. Differential privacy guarantees privacy by ensuring that the participation of a single individual in a dataset does not significantly affect the probability of any outcome; this is enforced by adding enough noise to obscure the influence of a single person. 

To apply differential privacy to graph data, it is therefore important to determine what a single person's data contributes to the graph. Prior work has looked at two forms of differential privacy in graphs -- {\em{edge differential privacy}}, where an edge corresponds to a person's private value, and {\em{node differential privacy}}, where a single node corresponds to a person. In our motivating application, a patient corresponds to a node, and hence node differential privacy is our privacy notion of choice. 

Prior work on edge differential privacy~\cite{NRS07, hay2009accurate} has looked at how to compute a number of statistics for {\em{static graphs}} while preserving privacy. For example,~\cite{karwa2011private} computes subgraph counts, and~\cite{hay2009accurate} degree distributions with edge differential privacy. It is also known how to successfully calculate more complex graph parameters under this notion; for example,~\cite{lu2014exponential} fits exponential random graph models and~\cite{wang2013differential, ahmed2013random} computes spectral graph statistics such as pagerank. 

In contrast, achieving node differential privacy is considerably more challenging. Changing a single node and its associated edges can alter even simple statistics of a static graph significantly; this means that any differentially private solution needs to add a considerable amount of noise to hide the effect of a single node, resulting in low utility. Prior work has addressed this challenge in two separate ways. The first is to assume that there is a publicly known upper bound on the maximum degree of any node in the graph~\cite{borgs2015private, gehrke2011towards}. 

The second is to use a carefully-designed projection from the input graph to a bounded degree graph, where adding or removing a single node has less effect, and then release statistics of the projected graph with privacy. To ensure that the entire process is privacy-preserving, the projection itself is required to be {\em{smooth}} -- in the sense that changing a single node should not change the statistics of the projected graph by much. This approach has been taken by~\cite{kasiviswanathan2013analyzing}, who releases degree distributions and subgraph counts for static graphs and~\cite{blocki2013differentially}, who releases subgraph counts and local profile queries. \cite{raskhodnikova2015efficient} releases degree distributions by using a flow-based projection algorithm. Finally, ~\cite{day2016publishing} proposes an improved projection method for releasing degree distributions, and is the state-of-the-art in this area. In this paper, we show that when the graph arrives {\em{online}}, existing projection-based approaches can yield poor utility, and therefore, we consider bounded degree graphs, where domain knowledge suggests an upper bound on the maximum degree.



%

%

%





%
%
%
%
%

%

%
%
%
%
%
%
%
%
%
%
%
%

Finally, while we are not aware of any work on differentially private statistics on streaming graph data, prior work has looked at releasing private statistics on streaming {\em{tabular data}} in an online manner~\cite{bolot2013private, cao2013efficient, chan2011private, kellaris2014differentially, chen2017pegasus, dwork2010differential}. In these settings, however, complete information about a single person (or a group of people) arrives at each time step, which makes the problem of private release considerably easier than online graph data, where newly arriving nodes may include information in the form of edges to already existing nodes. Thus, these approaches do not directly translate to online graphs. 


%
%









==> untitled folder/macro.tex <==
%
\usepackage[margin=1in]{geometry}
%
\usepackage{times}
%
\usepackage{graphicx} %
%
\usepackage{subcaption} 
\usepackage{caption}
\usepackage{tabularx}
\usepackage{lipsum}

%
%

%
\usepackage{hyperref}
\usepackage{url}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{enumerate}%


\usepackage{algorithm}
%
\usepackage{algpseudocode}
%


\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\Lap}[1]{\text{Lap}\left(#1\right)}
\newcommand{\card}[1]{\texttt{card}(#1)}

\usepackage[usenames, dvipsnames]{color}
\usepackage{tikz}
\usetikzlibrary{arrows}


%
%
%
%
\newcommand{\showinlater}[1]{}


\newcommand{\rmk}[1]{{\textcolor{ForestGreen}{RMK: #1}}}
\newcommand{\notshow}[1]{}
\def\calS{\mathcal{S}}
\def\calQ{\mathcal{Q}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}

\newcommand{\Dinf}[2]{D_{\infty}\big(#1 ~\|~ #2\big)}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{condition}[theorem]{Condition}

\renewcommand{\Pr}[2]{\mathbb{P}_{#1}\left[ #2 \right]}
\renewcommand{\exp}[1]{\text{exp}\left( #1 \right)}
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[ #2 \right]}
\newcommand{\KL}[2]{D_{\text{KL}} \left(#1 \| #2\right)}
\newcommand{\erf}[1]{\text{erf} \left(#1 \right)}



\newcommand{\new}{\text{new}}
\newcommand{\old}{\text{old}}
\newcommand{\edi}{\text{date}}


\newcommand{\plus}[1]{\left(#1\right)_{+}}

\usepackage{bbm}
\newcommand{\ind}[1]{\mathbbm{1}\left(#1\right)}
\newcommand{\tri}[1]{\triangle\left(#1\right)}
\newcommand{\Dmax}{D_{\max}}

\newcommand{\nodeprivacy}{%
\ifnum\spacefactor=3000
\expandafter\MakeUppercase\fi%
node differential privacy}

\def\calG{\mathcal{G}}
\def\calA{\mathcal{A}}
\def\calT{\mathcal{T}}

\def\tC{\tilde{C}}

\renewcommand{\deg}{\text{deg}}
\newcommand{\degree}[2]{\deg_{#1}\left(#2\right)}
\newcommand{\outdegree}[2]{\text{out-}\deg_{#1}\left(#2\right)}
\newcommand{\indegree}[2]{\text{in-}\deg_{#1}\left(#2\right)}

\newcommand{\edge}[2]{\text{edge}_{#1}\left(#2\right)}
\newcommand{\outedge}[2]{\text{out-edge}_{#1}\left(#2\right)}
\newcommand{\inedge}[2]{\text{in-edge}_{#1}\left(#2\right)}
\newcommand{\numedge}[2]{\text{numedge}_{#1}\left(#2\right)}

\newcommand{\Din}{D_{\text{in}}}
\newcommand{\Dout}{D_{\text{out}}}
\def\tD{\tilde{D}}
\def\tDin{\tilde{D}_{\text{in}}}
\def\tDout{\tilde{D}_{\text{out}}}


\newcommand{\highdegree}[2]{\text{highDeg}_{#1}\left(#2\right)}
\newcommand{\highoutdegree}[2]{\text{highOutDeg}_{#1}\left(#2\right)}

\newcommand{\hist}[1]{\text{hist}\left(#1\right)}
\newcommand{\histout}[1]{\text{histOut}\left(#1\right)}

\newcommand{\cross}[2]{\text{cr}_{#1}\left(#2\right)}


\newcommand{\GS}[2]{\text{GS}_{#1}\left(#2\right)}

\newcommand{\kstar}[3]{\star^{#1}_{#2}\left(#3\right)}
\newcommand{\numkstar}[2]{\star^{#1}\left(#2\right)}
\renewcommand{\tri}[2]{\triangle_{#1}\left(#2\right)}
\renewcommand{\S}[2]{S_{#1}\left(#2\right)}
\newcommand{\f}[1]{f\left(#1\right)}

\newcommand{\rom}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
%

%
%
%
\makeatletter
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}
%
%
%
%

\def\Elater{E_{\text{later}}}
\newcommand{\seq}[3]{\left(#1\right)_{#2}^{#3}}
\newcommand{\paren}[1]{\left(#1\right)}

\def\time{\texttt{time}}


\def\argmin{\text{argmin}}
\def\argmax{\text{argmax}}
\input{macro_shapes}


%
\def\sensdiff{\textsc{SensDiff}}
\def\composeD{\textsc{Compose-$D$-bounded}}
\def\composeproj{\textsc{Compose-projection}}
\def\sensseqD{\textsc{SensSeq-$D$-bounded}}
\def\sensseqproj{\textsc{SensSeq-projection}}
%

\newcommand{\bigO}[1]{\ensuremath{O\left(#1\right)}}
\newcommand{\Var}[1]{\ensuremath{\mathrm{Var}\left(#1\right)}}



==> untitled folder/macro_shapes.tex <==
\newcommand\shapescale{7}
\newcommand\starscale{4}
\newcommand\shapenodesize{1.5pt}
\tikzset{vertex/.style = {shape=circle,fill=black,inner sep=0pt,draw,minimum size=\shapenodesize}}
\tikzset{dedge/.style = {->,> = latex'}}
\tikzset{edge/.style = {-,> = latex'}}

\newcommand{\udtriangle}{
\begin{tikzpicture}
%
\node[vertex] (a) at  (0,0) {};
\node[vertex] (b) at  (-1/\shapescale,-1.73/\shapescale) {};
\node[vertex] (c) at  (1/\shapescale, -1.73/\shapescale) {};
%
\draw[edge] (a) to (b);
\draw[edge] (b) to (c);
\draw[edge] (a) to (c);
\end{tikzpicture}
}
\newcommand{\dtriangleI}{
\begin{tikzpicture}
%
\node[vertex] (a) at  (0,0) {};
\node[vertex] (b) at  (-1/\shapescale,-1.73/\shapescale) {};
\node[vertex] (c) at  (1/\shapescale, -1.73/\shapescale) {};
%
\draw[dedge] (a) to (b);
\draw[dedge] (b) to (c);
\draw[dedge] (c) to (a);
\end{tikzpicture}
}
\newcommand{\dtriangleII}{
\begin{tikzpicture}
%
\node[vertex] (a) at  (0,0) {};
\node[vertex] (b) at  (-1/\shapescale,-1.73/\shapescale) {};
\node[vertex] (c) at  (1/\shapescale, -1.73/\shapescale) {};
%
\draw[dedge] (a) to (b);
\draw[dedge] (b) to (c);
\draw[dedge] (a) to (c);
\end{tikzpicture}
}


\newcommand{\dstarI}{
\begin{tikzpicture}
%
\node[vertex] (a) at  (0,0) {};
\node[vertex] (b) at  (0,  1/\starscale) {};
\node[vertex] (c) at  (0, -1/\starscale) {};
\node[vertex] (d) at  (-1/\starscale, 0) {};
\node[vertex] (e) at  (1/\starscale, 0) {};
%
\draw[dedge] (a) to (b);
\draw[dedge] (a) to (c);
\draw[dedge] (a) to (d);
\draw[dedge] (a) to (e);
\end{tikzpicture}
}
\newcommand{\dstarII}{
\begin{tikzpicture}
%
\node[vertex] (a) at  (0,0) {};
\node[vertex] (b) at  (0,  1/\starscale) {};
\node[vertex] (c) at  (0, -1/\starscale) {};
\node[vertex] (d) at  (-1/\starscale, 0) {};
\node[vertex] (e) at  (1/\starscale, 0) {};
%
\draw[dedge] (b) to (a);
\draw[dedge] (c) to (a);
\draw[dedge] (d) to (a);
\draw[dedge] (e) to (a);
\end{tikzpicture}
}
\newcommand{\udstar}{
\begin{tikzpicture}
%
\node[vertex] (a) at  (0,0) {};
\node[vertex] (b) at  (0,  1/\starscale) {};
\node[vertex] (c) at  (0, -1/\starscale) {};
\node[vertex] (d) at  (-1/\starscale, 0) {};
\node[vertex] (e) at  (1/\starscale, 0) {};
%
\draw[edge] (b) to (a);
\draw[edge] (c) to (a);
\draw[edge] (d) to (a);
\draw[edge] (e) to (a);
\end{tikzpicture}
}
\newcommand{\udkstar}[1]{\ensuremath{\udstar_{#1}}}
\newcommand{\dkstarI}[1]{\ensuremath{\dstarI_{#1}}}
\newcommand{\dkstarII}[1]{\ensuremath{\dstarII_{#1}}}


\newcommand{\dedge}{
\begin{tikzpicture}
%
\node[vertex] (a) at  (0,0) {};
\node[vertex] (b) at  (2/\shapescale, 0) {};
%
\draw[dedge] (a) to (b);
\end{tikzpicture}
}
\newcommand{\udedge}{
\begin{tikzpicture}
%
\node[vertex] (a) at  (0,0) {};
\node[vertex] (b) at  (2/\shapescale, 0) {};
%
\draw[edge] (a) to (b);
\end{tikzpicture}
}



==> untitled folder/metaalg.tex <==
\section{Main Algorithm}\label{sec:main_alg}

Recall that we are given as input a $D$-bounded (or $(\Din, \Dout)$-bounded) graph sequence $\calG = ( G_1, G_2, \ldots, G_T )$ that arrives online, a privacy budget $\epsilon$ and a function $f$. Our goal is to publish an $\epsilon$-differentially private approximation to the sequence $f(\calG)$ in an online manner. Specifically, at time $t$, an incoming vertex set $\partial{V_t}$ and edges $\partial{E_t}$ adjacent to it and the existing vertices arrive, and our goal is to release a private approximation to $f(G_t)$ with low additive $L_1$-error. 

\paragraph{Baseline Approaches.} A naive approach is to calculate $f(G_t)$ at each $t$ and add noise proportional to its global sensitivity over $\epsilon$. Since $\partial{E_t}$ may contain information on individuals in $G_{t-1}$ in the form of adjacent edges, this procedure will not provide $\epsilon$-differential privacy. 

The correct way to do privacy accounting for this method is by sequential composition~\cite{DMNS06}. Suppose the graph sequence has total length $T$ and we allocate privacy budget $\epsilon/T$ to each time step; then at time $t$, we calculate $f(G_t)$ and add noise proportional to its global sensitivity divided by $\epsilon/T$. If the global sensitivity of $f(G_t)$ is $O(1)$, then, we add $O(T/\epsilon)$ noise to $f(G_t)$, which results in a $\Theta(T^2/\epsilon)$  expected $L_1$-error between $f(\calG)$ and the output of the algorithm. 

A second approach is to calculate $f(G_t)$ and add noise proportional to the global sensitivity of the (entire) sequence $f(\calG)$ divided by $\epsilon$. This preserves $\epsilon$-differential privacy. However, the global sensitivity of the sequence $f(\calG)$ typically grows linearly with $T$, the length of the entire graph sequence, even if the graph sequence itself is degree-bounded. For example, if $f(G)$ is the number of nodes in $G$ with degree $\geq \tau$, then, a single extra node with degree $\tau + 1$, added at time $t=1$, can increase $f(G_t)$ by $1$ for {\em{every}} $t$, resulting in a global sensitivity of $\Omega(T)$. Consequently, the expected $L_1$-error between the true value of $f(\calG)$ and the output of this approach is as again large as $\Theta(T^2/\epsilon)$. 

%
%

%

\paragraph{Our Approach.} The main observation in this work is that for a number of popular functions, the {\em{difference sequence}} $\Delta = ( f(G_1), f(G_2) - f(G_1), f(G_3) - f(G_2), \ldots)$ has considerably better properties. Observe that unlike certain functions on tabular data \cite{bolot2013private, cao2013efficient, chan2011private, kellaris2014differentially, chen2017pegasus, dwork2010differential}, releasing $f(G_t) - f(G_{t-1})$ after adding noise proportional to its sensitivity over $\epsilon$ will still not be $\epsilon$-differentially private -- this is because $\partial{E_t}$ can still include edges adjacent to people in $G_{t-1}$. 

However, the difference sequence $\Delta$ does have  considerably less global sensitivity than $f(\calG)$. In particular, we show that if the graph sequence $\calG$ is $D$-bounded, then, the global sensitivity $\GS{}{\Delta}$ of the entire difference sequence for a number of popular functions $f$ depends only on $D$ and not on the sequence length $T$. For example, in Section~\ref{sec:highdeg}, we show that when $G$ is an undirected graph and $f$ is the number of nodes with degree $\geq \tau$, the global sensitivity of the entire difference sequence is at most $2D + 1$. 

This immediately suggests the following algorithm.  At time $t$, calculate the difference $\Delta_t = f(G_t) - f(G_{t-1})$, and add Laplace noise proportional to its global sensitivity over $\epsilon$ to get a private perturbed version $\tilde{\Delta}_t$. Release the partial sum $\sum_{s=1}^{t} \tilde{\Delta}_s$, which is an approximation to $f(G_t)$. Since the expected value of $\tilde{\Delta}_t - \Delta_t$ is independent of $T$, the maximum standard deviation of any partial sum is at most $O(\sqrt{T}/\epsilon)$, which results in an expected $L_1$-error of $O(T^{3/2}/\epsilon)$ -- better than the $O(T^2/\epsilon)$-error achieved by the two baseline approaches. 

%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%

\begin{algorithm}[h]
\caption{\sensdiff(Graph sequence $\calG$, query $f$, privacy parameter $\epsilon$)}
\label{alg}
\begin{algorithmic}
\For{$t=1, \ldots, T$}
\State{Receive $\partial{V_t}$ and $\partial{E_t}$, and construct $G_t$.}
\State{Calculate $\Delta_t = f(G_t) - f(G_{t-1})$.}
\State{Let $\GS{D}{\Delta}$ be the global sensitivity of the difference sequence;}
\State{Calculate $\tilde{\Delta}_t = \Delta_t + \Lap{\frac{\GS{D}{\Delta}}{\epsilon}}$, and the partial sum $\sum_{s=1}^{t} \tilde{\Delta}_s$.}
\EndFor
\State{\textbf{return} $\seq{\sum_{s=1}^{t} \tilde{\Delta}_s}{t=1}{T}$}
\end{algorithmic}
\end{algorithm}


The full algorithm, applied to a generic function $f$, is described in Algorithm~\ref{alg}. We call it \sensdiff\ as it uses the global sensitivity of the difference sequence $\Delta$.
The rest of the paper is devoted to analyzing the global sensitivity of the difference sequence for a number of popular graph functions $f$. Our analysis exploits specific combinatorial properties of the graph functions in question, and is carried out for two popular classes of graph functions -- functions of the degree distribution and subgraph counts. 

%





==> untitled folder/metaalgoffline.tex <==
\section{The Main Algorithm}

We now consider the main problem of this paper. We are given a $D$-bounded graph sequence $\calG = ( G_1, G_2, \ldots )$, a privacy parameter $\epsilon$ and a function $f$ and our goal is to publish an approximation to the sequence $f(\calG)$. We also assume that the graph sequence arrives in an online manner as nodes get added; this implies that at time $t$, we only have access to $(G_1, G_2, \ldots, G_t)$. 

A naive approach to this problem is as follows. For each $t$, calculate $f(G_t)$ and add noise proportional to the global sensitivity divided by $\epsilon$. Unfortunately, it so happens that for many popular functions $f$, the global sensitivity scales with $m$, the length of the entire graph sequence even if it is degree-bounded. For example, suppose $f(G)$ is the number of nodes in $G$ with degree $\geq \tau$. Here, a single extra node with degree $\geq \tau$, added at time $t=1$, can increase $f(G_t)$ by $1$ for {\em{every}} $t$, thus increasing the global sensitivity of the sequence by $m$. 

The main observation in this work is that for a lot of popular functions $f$, the {\em{difference sequence}} $( f(G_1), f(G_2) - f(G_1), f(G_3) - f(G_2), \ldots)$ has considerably less global sensitivity. In particular, we show that if the graph sequence $\calG$ is $D$-bounded, for a number of functions $f$, the global sensitivity $\GS{D}{\Delta}$ of the entire difference sequence depends only on $D$ and not on the sequence length $m$. For example, in Section~\ref{sec:highdeg}, we show that if $f$ is the number of nodes with degree $\geq \tau$, then the global sensitivity of the entire sequence is at most $2D + 1$ for $D \geq \tau$. 

This immediately suggests the following algorithm.  For each $t \geq 1$, calculate the difference sequence $(\Delta_t)$, and add Laplace noise proportional to its global sensitivity over $\epsilon$ to get a private perturbed version $\tilde{\Delta}_t$. Then, the partial sums $(\tilde{\Delta}_1, \tilde{\Delta}_1 + \tilde{\Delta}_2, \ldots )$ constitute an approximation to $f(\calG)$ Observe that at time $t$, we only need to access the sequence $G_1, \ldots, G_t$, so the entire algorithm can be run online. Algorithm~\ref{alg} describes a general version of the algorithm, applied to a generic function $f$.


\begin{algorithm}[H]
\KwIn{Graph sequence $\calG$, query $f$, privacy parameter $\epsilon$}
Calculate the difference sequence $(\Delta)$, where $\Delta_1 = f(G_1)$, $\Delta_t = f(G_t) - f(G_{t-1})$, for $t \geq 1$.\\ 
Let $\GS{D}{\Delta}$ be the global sensitivity of the difference sequence\;
Calculate $\tilde{\Delta}_t = \Delta_t + \Lap{\frac{\GS{D}{\Delta}}{\epsilon}}$, for $t=1, \ldots, m$.\\
\Return{$\{ \sum_{s=1}^{t} \tilde{\Delta}_s \}_{t=1}^m$}
\caption{Main algorithm for publishing a function of a graph sequence}
\label{alg}
\end{algorithm}

The rest of the paper is devoted to analyzing the global sensitivity of the difference sequence for a number of popular functions $f$, and showing that it is independent of $m$.

\kc{One thing that does not come across -- what about composition? Think about how to write this properly.}



==> untitled folder/preliminaries.tex <==
\section{Preliminaries}

\subsection{Graphs and Graph Sequences}\label{sec:into_graph}

Formally, we consider a graph $G = (V, E)$, where a node $v \in V$ represents a person and an edge $(u, v) \in E$ a relationship. $G$ may be directed or undirected, depending on the application. We assume that each node $v \in V$ is associated with a time stamp, denoted by $v.\time$, that records when $v$ enters the graph.

In our setting, a graph arrives online as more and more of its vertices and some of their adjacent edges become visible. More specifically, at time $t$, a set of vertices $\partial{V_t}$ arrives, along with a set of edges $\partial{E_t}$; each edge in $\partial{E_t}$ has at least one end-point in $\partial{V_t}$, and the other end-point may be a vertex that arrived earlier. These vertices and edges, along with vertices and edges that arrived earlier comprise a graph $G_t$. Given a function $f$ that operates on graphs, our goal is to output (a private approximation to) $f(G_t)$ at each time step $t$.

More formally, the arrival process comprises a {\em{graph sequence}} $\calG = (G_1, G_2, \ldots)$, which is defined as a sequence of graphs with $G_t = (V_t, E_t)$ such that $V_0 = \emptyset$, $\partial{V_t} =  \{ v: v.\time = t \}$ is the set of all nodes with time stamp $t$ and $V_t = V_{t-1} \cup \partial {V_t}$ for $t \geq 1$ is the set of all nodes with time stamps $\leq t$.
Additionally, we let $E_0 = \emptyset$, 
$ \partial{E_t} = \{ (u, v) | u \in \partial{V_t}, v \in V_t  {\text{\ or\ }} u \in V_t, v \in \partial{V_t}\}$, 
and $E_t = E_{t-1} \cup \partial{E_t}$. Given a function $f$ that operates on a graph, we define $f$ applied to the graph sequence $f(\calG)$ as the sequence $(f(G_1), f(G_2), \ldots)$. 

If the graph sequence is $\calG = (G_1, G_2, \ldots, G_T)$, then the error of $\calA(G)$ is defined as: $\sum_{t=1}^{T} | \calA(G_t) - f(G_t)|$. Our goal is to design an algorithm $\calA$ that has as low error as possible. 



\subsection{Differential Privacy}\label{sec:dp}

The gold standard for privacy in data-mining applications is differential privacy~\cite{DMNS06}, which essentially ensures that the participation of a single person in a database does not change the probability of any outcome by much. The formal definition is as follows. 

%
%

\begin{definition}[$\epsilon$-Differential privacy]
A randomized algorithm $\calA$ is said to guarantee $\epsilon$-differential privacy if for any two databases $S$ and $S'$ that differ in the private value of a single individual, and for any $w \in \text{Range}(\calA)$, we have
\begin{align*}
\Pr{}{\calA(S) = w} \leq e^{\epsilon} \cdot \Pr{}{\calA(S') = w},
\end{align*}
where the probability is with respect to the randomness in $\calA$. Here $\epsilon$ is a privacy parameter, often called the {\em{privacy budget}}. 

\end{definition}

\paragraph{Global Sensitivity Mechanism.} A popular differential privacy mechanism is the Global Sensitivity Mechanism, introduced by~\cite{DMNS06}. Let $f$ be a function that operates on a database $S$. The Global Sensitivity of $f$, denoted by $\GS{}{f}$, is the maximum value of the difference $\| f(S) - f(S') \|_1$ when $S$ and $S'$ are any two databases that differ by a the participation of a single person. 

Given a function $f$, a database $S$ and a privacy budget $\epsilon$, the Global Sensitivity Mechanism computes an $\epsilon$-differentially private approximation to $f(S)$ as follows: $\calA_{GS}(S) = f(S) + \Lap{\frac{\GS{}{f}}{\epsilon}}.$ It was shown in~\cite{DMNS06} that this method preserves $\epsilon$-differential privacy. 

\paragraph{Node Differential Privacy.} To apply differential privacy to graphs, we need to determine what constitutes a single person's data in a graph. For the kind of graphs that we will study, a node $v$ corresponds to a single person. This is known as {\em{node differential privacy}}~\cite{hay2009accurate}, %
which ensures that the addition or removal of a single node along with its adjacent edges does not change the probability of any outcome by much. 


%

%
%
%
%
%
%

%
%
%
%
%
%
%



%
%
%
%

%

%
%
%
%

%
%
%
%
%
%

%
%
%
%
%
%
%

%
%
%
%
%
%
%
%

\subsection{Bounded Degree Graphs}


A major challenge with ensuring node differential privacy is that the global sensitivity $\GS{}{f}$ may be very large even for simple graph functions $f$, which in turn requires the addition of a large amount of noise to ensure privacy. For example, if $f$ is the number of nodes with degree $\geq 1$, and we have an empty graph $G$ on $n$ nodes, then adding a single node connected to every other node can increase $f$ by as much as $n$. 

%
%

Prior work has addressed this challenge in two separate ways. The first is by considering {\em{Bounded Degree Graphs}} \cite{kasiviswanathan2013analyzing, blocki2013differentially, borgs2015private}, where an a-priori bound on the degree of any node is known to the user and the algorithm designer. This is the solution that we will consider in this paper. 

A second line of prior work ~\cite{blocki2013differentially, kasiviswanathan2013analyzing, raskhodnikova2015efficient, day2016publishing} 
%
presents {\em{Graph Projections}} algorithms
that may be used to project graphs into lower degree graphs such that the resulting projections have low global sensitivity for some graph functions.  In Section~\ref{sec:highdeg}, we show that natural extensions of some of these projections may be quite unstable when a graph appears online. 

We first define bounded degree graphs.
Let $\degree{G}{v}$ denote the degree of node $v$ in an undirected graph $G$, $\outdegree{G}{v}$ and $\indegree{G}{v}$ denote the out-degree and in-degree of $v$ in a directed graph $G$.
\begin{definition}\label{def:D-bdd}
An undirected graph $G = (V, E)$ is $D$-bounded if $\degree{G}{v}\leq D$ for any $v\in V$. 
A graph sequence $\calG = (G_1, G_2, \ldots)$ is $D$-bounded if for all $t$, $G_t$ is $D$-bounded. %
In other words, the degree of all nodes remain bounded by $D$ in the entire graph sequence. 

A directed graph $G = (V, E)$ is $\Dout$-out-bounded if $\outdegree{G}{v}\leq \Dout$ for any $v\in V$. 
A graph sequence $\calG = (G_1, G_2, \ldots)$ is $\Dout$-out-bounded if for all $t$, $G_t$ is $\Dout$-out-bounded. %
%
Similarly, $G$ is $\Din$-in-bounded if $\indegree{G}{v}\leq \Din$ for any $v\in V$. $\calG$ is $\Din$-in-bounded if for all $t$, $G_t$ is $\Din$-in-bounded.

We say a directed graph or a graph sequence is $(\Din, \Dout)$-bounded if it is both $\Din$-in-bounded and $\Dout$-out-bounded.
\end{definition}

In this work, we assume that the domain consists only of degree bounded graphs. This ensures that the global sensitivity of certain common graph functions, such as degree distribution and subgraph counts, is low, and allows us to obtain privacy with relatively low noise. Additionally, many common sensitive graphs, such as the HIV transmission graph and co-authorship networks, typically have relatively low maximum degree, thus ensuring that the assumption holds for low or moderate values of $D$. 





%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%


%

%
%
%
%
%

%

%
%
%
%
%
%

%
%
%
%
%
%
%
%

%
%
%
%
%
%
%

%

%


%

%
%
%
%
%
%

%
%
%

%
%


\subsection{Graph Functions}

This work will consider two types of functions on graph sequences. The first consists of functions of the degree distribution. The specific functions we will look at for undirected graphs are $\highdegree{\tau}{G}$, which counts the number of nodes in $G$ with degree $\geq \tau$ and the degree histogram $\hist{G}$, which counts the number of nodes with degree $d$ for any $d \in \mathbb{N}_{+}$.
%
%
Similarly, for directed graph, we consider $\highoutdegree{\tau}{G}$, the number of nodes with out-degree $\geq \tau$, and the out-degree histogram $\histout{G}$, which counts the number of nodes with out-degree $d$ for any $d \in \mathbb{N}_{+}$.
%

%
%

%

The second class of functions will involve subgraph counts. Given a subgraph $S$, we will count the number of occurrences of this subgraph $\S{}{G}$ in the entire graph $G$. For example, when $S$ is a triangle, $\S{}{G}$ will count the number of triangles in the graph. When $G$ is directed, so will be the corresponding subgraphs. 

\subsection{Other Notations}\label{sec:notation}

%
%

%

%

%
%
In a directed graph, an edge is denoted by an ordered tuple, i.e., $(u, v)$ represents a directed edge pointing from node $u$ to $v$. 

%
%

%

%

We use $\seq{a_t}{t = 1}{T}$ as an abbreviation for vector $(a_1, a_2, \dots, a_T)$.
%

For any integer $i$, we use $[i]$ to denote the set $\{1,2,\dots,i\}$.

A degree histogram $h$ is a mapping from degrees to counts, i.e., given $d \in \mathbb{N}_{+}$, $h(d)$ is the number of nodes with degree equal to $d$. 
%
We define the distance between two histograms $h$ and $h'$ as $\|h(d) - h'(d)\|_1 = \sum_{d\in\mathbb{N}_{+}} |h(d) - h'(d)|$.
Given two sequences of histograms 
$\seq{h_t}{t=1}{T}$ and $\seq{h'_t}{t=1}{T}$, 
%
we define the generalized $L_1$ distance between them as $\sum_{t = 1}^T \|h_t(d) - h'_t(d)\|_1$.


